Toward Micro-Dialect Identification in Diaglossic and Code-Switched Environments

Although the prediction of dialects is an important language processing task, with a wide range of applications, existing work is largely limited to coarse-grained varieties. Inspired by geolocation research, we propose the novel task of Micro-Dialect Identification (MDI) and introduce MARBERT, a new language model with striking abilities to predict a fine-grained variety (as small as that of a city) given a single, short message. For modeling, we offer a range of novel spatially and linguistically-motivated multi-task learning models. To showcase the utility of our models, we introduce a new, large-scale dataset of Arabic micro-varieties (low-resource) suited to our tasks. MARBERT predicts micro-dialects with 9.9% F1, ~76X better than a majority class baseline. Our new language model also establishes new state-of-the-art on several external tasks.

==> approach.tex <==
%\subsection*{Approach}\label{subsec:approach}
%-------------


\textbf{Context.} In spite of the importance of language technologies, the great majority of the world's currently known 7,111 living languages~\footnote{Source: \url{https://www.ethnologue.com}.} are not yet NLP-supported. As technology continues to play an increasingly impactful role in our lives, access to nuanced NLP tools (including MDI) becomes an issue of equity~\cite{jurgens2017incorporating}. Practically, it is still challenging to find tools for closely related languages and varieties, including those that are widely spoken. We focus on one such situation for the Arabic language, a large collection of similar varieties with $\sim$ 400 million native speakers. For Arabic, currently available NLP tools are limited to the standard variety of the language, Modern Standard Arabic (MSA), and a small set of dialects such as Egyptian, Levantine, and Iraqi. Arabic dialects differ amongst themselves and from MSA at various levels, including phonological and morphological~\cite{watson2007phonology}, lexical~\cite{salameh2018fine,mageedYouTweet2018,qwaider2018shami}, syntactic~\cite{benmamoun2011agreement}, and sociological~\cite{bassiouney2009arabic,bassiouney2017identity}. 

A major limitation to developing robust and equitable language technologies for Arabic has been absence of large, diverse data. A number of pioneering efforts, including shared tasks~\citep{zampieri2014report,malmasi2016discriminating,zampieri2018language}, have been invested to bridge this gap by collecting datasets. However, these works either depend on automatic geocoding of user profiles~\citep{mageedYouTweet2018}, which is not quite accurate, as we show in Section~\ref{sec:data_acq}, use a small set of dialectal seed words as a basis for the collection~\citep{zaghouani2018arap,qwaider2018shami}, which limits text diversity, or are based on translation of a small dataset of sentences rather than naturally-occurring text~\cite{salameh2018fine}. 


%\textbf{Context.} We carry out our study on Arabic, a language of $\sim 400$M native speakers with a wide range of dialects covering an extensive geographical region across Asia and Africa. 

Other motivations for choosing Arabic as the primary context of our work is that Arabic is diaglossic language, with a so-called `high' variety (used in educational and formal settings) and `low' variety (used in everyday communication). This allows us to exploit dialgossia in our models. For historical reasons, different foreign languages are used in code-switching settings by different people in the Arab world (e.g., English in Egypt, French in Algeria, Italian in Libya). Our choice of Arabic thus allows us to also test the effect of integrating code-switching in our models.  

-- Collect and label a high-quality dataset

-- Develop supervised and semi-supervised models, employing a novel MTL approach.

-- Introduce a powerful language model for Arabic dialects

-- Exploit code-switching and diaglossia to enhance classification



==> bert.tex <==

\subsection{BERT}\label{subsec:bert}
%-----------------
BERT~\cite{devlin2018bert} stands for \textbf{B}idirectional \textbf{E}ncoder \textbf{R}epresentations from \textbf{T}ransformers. It is an approach for pre-training language representations that involves two unsupervised learning tasks, (1) \textit{masked language models (Masked LM)} and (2) \textit{next sentence prediction}. Since BERT uses bidirectional conditioning, a given percentage of random input tokens are masked and the model attempts to predict these masked tokens. 
.~\citet{devlin2018bert} mask 15\% of the tokens (the authors use \textit{word pieces}) and feed the final hidden vectors of these masked tokens to an output softmax over the vocabulary. The next sentence prediction task of BERT is also straightforward.~\citet{devlin2018bert} simply cast the task as binary classification. For a given sentence \texttt{S}, two sentences \texttt{A} and \texttt{B} are generated where \texttt{A} (positive class) is an actual sentence from the corpus and \texttt{B} is a randomly chosen sentence (negative class). Once trained on an unlabeled dataset, BERT can then be fine-tuned with supervised data.


==> geo.tex <==
\section{Geolocation}\label{sec:geo}
We exploit our novel GEO-ARA dataset to model geolocation. For this purpose, we use a single task BERT to predict geolocation at the tweet level and then port performance at the use-level by taking the majority class over user tweets. We only consider tweets predicted with $0.35$ in the softmax layer. We follow the literature in reporting acc, acc@161 (classification accuracy within a circle or radius of 100 miles/161 kiolemters from the center of the gold city), mean and media error (measured in kilometers between the predicted and true city). Our model acquires 15.27\% acc, 23.74\% acc@161, 1100.25km mean distance, and 788.75km median distance.~\footnote{The message-level geolocation model is at 6.70\% acc, 4.42\% $F_1$, 15.40\% acc@161, 1152.04 km mean distance,	827.90km media distance.} A baseline model that does not exploit the softmax value on this task only acquires 11.86\% acc.%0.08128363557480436 

% f1: 0.08128363557480436
% acc: 0.11868131868131868



==> impact.tex <==
\section{Impact of our Data and Models}\label{sec:impact}
%----------------


%---------------
In this section, we showcase 3 main scenarios where our data and models can have a significant impact. \textbf{(1)} We exploit the \textit{noisy-labeled} data in our wider collection to improve our dialect id (country) models (Section~\ref{subsec:noisy}). \textbf{(2)} We use a large subset of our \textit{unlabeled} data to develop a powerful language model and show its superior performance on several external tasks, as well as our MDI tasks (Section~\ref{subsec:marabert}). \textbf{(3)} We demonstrate how sample external text classification tasks (e.g., sentiment analysis) can benefits when trained in a multi-task settings with one of our \textit{models} (Section~\ref{subsec:transfer}). 


\subsection{Learning From Noisy Labels}\label{subsec:noisy}
%------------------------


\begin{table}[h]
\centering
\footnotesize 
\begin{tabular}{lll} \hline 
\textbf{Supervision} & \textbf{acc} & \textbf{F1} \\ \hline 
%	
Baseline I (majority in TRAIN)  & 9.21 & 0.84 \\
Baseline II (Gold) & 46.84 & 37.64 \\ \hline
Weak & 41.17 & 23.70 \\
Weak+Gold & \textbf{49.77} & 38.25 \\
Weak\_\textit{then}\_Gold & 47.86 & \textbf{38.56}\\ \hline
\end{tabular}%
\caption{Results on TEST with models exploiting noisy labels on 20 countries (with Djibouti excluded, and hence Baseline II [Gold] is slightly different from that reported in Table~\ref{tab:sprvsd_eval}). For comparison, our gold (BERT trained on human-labeled TRAIN) is re-trained with 20 classes.} 
\label{tab:noisy_res}
\end{table}
%-------------
In contrast to our gold-supervised models (Section~\ref{sec:sup_exps}), this set of experiments is focused on learning from noisy labels. We only perform experiments on predicting \textit{country} labels. Our goal is to answer the question ``To what extent can automatically acquired labels in our dataset be beneficial for learning?". To this end, we remove human annotated users from our larger automatically labeled pool and use only data tagged with any of the 319 cities whose users we manually labeled. Keeping tweets with at least 3 Arabic words, we acquire 1,161,651 tweets from 3,195 users, across all countries except Djibouti (all whose users were already in our human annotation round). As such, we have 20 countries in this dataset and refer to it simply as \texttt{Auto-Tagged}. We exploit Auto-Tagged in 3 experimental settings, reporting results on our gold TEST in all 3 cases. The 3 settings are: \textbf{(1) Weakly Supervised:} Where fine-tune BERT exclusively on Auto-Tagged; (2) \textbf{Weak+Gold:} Where concatenate Auto-Tagged and our TRAIN (gold), shuffle the dataset, and fine-tune BERT on it; and (3) \textbf{Weak-\textit{Then}-Gold:} Where fine-tune BERT on Auto-Tagged \textit{first}, then resume fine-tuning on our human labeled data (TRAIN). Table~\ref{tab:noisy_res} shows \textbf{Weak+Gold} to improve 2.923\% acc over our \textbf{Gold} model (Baseline II), establishing the utility of using noisy labels on the country level. %These are our best country-level models. 


% \subsection{mAraBERT: A New Language Model}\label{subsec:marabert}
% %------------------------
% We extract 1 billion tweets from our unlabeled collection and use these to train a new powerful bidirectional language model from transformers, similar to BERT but without the next sentence prediction objective. We refer to our new model as mAraBERT, to indicate its ability to handle micor-Arabic varieties. We provide more details about how we train mAraBERT in supplementary material. As Table xxx shows, mAraBERT enables us to perform significantly batter not only on our 3 tasks (city, state, and country), but on a range on external tasks thereby showing its positive impact. 

% \textbf{Single tasks:
% }
% - Nizar dataset

% - AraNet sentiment

% - Offensive and HS


% \subsection{Transfer Learning With Our Models}\label{subsec:transfer}
% Our micro-dialectal dataset, MICRO-ARA, is diverse and we expect it to have a significant impact on several downstream tasks. To demonstrate this, we collect 15 different sentiment analysis datasets comprising both MSA and dialectal Arabic from~\newcite{abdul2012awatif,abdulla2013arabic,aly2013labr,abdul2014samar,nabil2015astd,salameh2015sentiment,kiritchenko2016semeval,rosenthal2017semeval,alomari2017arabic,mohammad2018semeval,baly2019arsentd}. We map the different labels on these datasets to ``positive" and ``negative" and discard other categories such as ``neutral" or ``mixed". We obtain a total of 126,766 samples, which we split into 80\% TRAIN, 10\%, DEV, and 10\% TEST. We then train a single task BERT for 15 epochs as a baseline and then a multi-task BERT with micro-dialect id (MICRO-ARA data at the city level) as an auxiliary task. We evaluate the best single task model on the sentiment TEST set and find it at 77.31\% acc and 76.67\% $F_1$. 
% Our multi-task model acquires a whole 7\% improvement in \textit{both} acc and $F_1$ (\%=84.26 and 83.36, respectively). Although we do not compare to individual models from previous works, we believe our multi-task sentiment model reported here achieves a new SOTA for Arabic sentiment analysis. %After all, we train on all publicly available data.








==> mtl.tex <==
%-----------------------------
\subsection{Multi-Task Learning}

% \begin{figure}[h]
% \centering
% \frame{\includegraphics[width=0.4\textwidth]{images/mtl_1}}
% \caption{Our BiGRU MTL network for city, state, and country. The three tasks share 2 hidden layers, with each task having its independent attention layer.}
% \label{fig:mtl_t_spec_attn}
% \end{figure}
% %-----------------
We investigate the utility of \textit{Multi-Task Learning} (MTL) for language ID. The intuition behind MTL is that many real-world tasks involve making predictions about closely related labels or outcomes. For related tasks, MTL helps achieve inductive transfer between the various tasks by leveraging additional sources of information from some of the tasks to improve performance on the target task~\cite{caruana1993}. By using training signals for related tasks, MTL allows a learner to prefer hypotheses that explain more than one task~\cite{caruana1997multitask} and also helps regularize models.
%In single task learning, an independent network is trained in isolation for each task. In contrast, in MTL, a number of tasks are learned together in a single network, with each task having its own output. An MTL network has a shared input, and one or more hidden layers that are shared between all the tasks. Backpropagation is then applied in parallel on all outputs. In our case, w
 Motivated by the promise of MTL, we train a single network for our city, state, and country tasks with one output for each of the three tasks. 
%  Figure ~\ref{fig:mtl_t_spec_attn} is an illustration of an MTL network for our 3 tasks for modeling dialect, with 2 shared hidden BiGRU layers and a task-specific (i.e., independent) BiGRU attention layer. In this model, each of the three tasks has its own loss function, with the MTL loss computed as:

% %-----------------
% \begin{equation}
% \begin{multlined}
%  \mathcal{L}(\theta_{MTL})\\= \left(\mathcal{L}(\theta_{city}) + \mathcal{L}(\theta_{state})+\mathcal{L}(\theta_{country}) \right) / 3 \\
%  \end{multlined}
% \end{equation}

%We now introduce the Transformer~\cite{vaswani2017attention}, since both our attention mechanism and BERT ~\cite{devlin2018bert} are based on it.


==> noisy_labels_learning.tex <==



==> semi-supervised_exps.tex <==
\section{Semi-Supervised Models}

\subsection{Self-Training with Unlabeled Data}
We employ self-training, a type of semi-supervised learning where a model is trained on gold labeled data and is used to tag a large amount of unlabeled data, with a goal to augment the gold training set with the most `\textit{confidently}' predicted cases. In our neural network models, we use the per-class value in the softmax layer as a confidence threshold. In other words, we consider tweets predicted above a given threshold `\textit{good enough}' and we use them to augment our training set. We run our self-training on a pool of 10M tweets (we refer to this set simply as \texttt{unlabeled}). \mam{explain how we extract this pool.} We have two settings for self-training with unlabeled data, \textit{(a) class-agnostic} and \textit{(b) class-specific}. For (a) class-agnostic, we add the top confidently predicted percentage of \texttt{unlabeled}, irrespective of the class assigned to a data point, to gold train. We experiment with top percentages from the set \textit{\{5\%, 10\%, 25\%\}}. For 
(b) class-specific, we add the top confidently predicted cases assigned to each class, again with values from the set \textit{\{5\%, 10\%, 25\%\}}. The class-specific setting ensures we get enough data from classes where the model tends not to be as highly confident as other classes dominating the training set. Table~\ref{tab:ssl_res} provides our results for the self-training experiments. \mam{This table should spell out all res across all self-traing exps, from this and next section}.

 \mam{describe how we acquire data for self-training. Describe including only tweets > 30/40? words length, only in direct addresses/replies between users, and with zero diacritics. \textbf{Importantly}, we can analyze the softmax values in the validation set, to get a per-class distribution over all tweets in dev.}





==> transformer.tex <==
\subsection{Transformer}\label{subsec:transformer}
The Transformer ~\citep{vaswani2017attention} is based solely on attention. Similar to most other sequence transduction models~\cite{bahdanau2014neural,cho2014learning,Sutskever2014SequenceTS}, it is an encoder-decoder architecture. It takes a sequence of symbol representations $x^{(i)} \dots x^{(n)}$, maps them into a sequence of continuous representations $z^{(i)} \dots x^{(n)}$ that are then used by the decoder to generate an output sequence $y^{(i)} \dots y^{(n)}$, one symbol at a time. This is performed using \textit{self-attention}, where different positions of a single sequence are related to one another. The Transformer employs an attention mechanism based on a function that operates on \textit{queries}, \textit{keys}, and \textit{values}. The attention function maps a query and a set of key-value pairs to an output, where the output is a weighted sum of the values. For each value, a weight is computed as a compatibility function of the query with the corresponding key. We implement and apply the multi-head attention function to our BiGRU models. 

\textit{Encoder} of the Transformer in~\citet{vaswani2017attention} has 6 attention layers, each of which is composed of two sub-layers: (1) \textit{multi-head attention} where, rather than performing a single attention function with queries, keys, and values, these are projected \textit{h} times into linear, learned projections and ultimately concatenated; and 
(2) fully-connected \textit{feed-forward network (FFN)} that is applied to each position separately and identically. 
\textit{Decoder} of the Transformer also employs 6 identical layers, similar to the encoder, yet with an extra/third sub-layer that performs multi-head attention over the encoder stack. 
As mentioned, the Transformer is the core learning component in BERT~\cite{devlin2018bert}, which we now introduce.




==> user_eval.tex <==
\section{Dialectal User-Level Evaluation}\label{sec:user_eval}
Our models are not designed to directly detect the dialect of a user, but rather takes a single tweet input at a time. However, we test how the model will fare on detecting user-level dialect given a set of tweets posted by the user. For the purpose, we train two models, one on MADAR data (shared tasks 1 and 2) and another on our MICRO-ARA+MADAR data. As Table~\ref{tab:external_eval} shows, our second model achieves a new SOTA on MADAR, outperforming the shared task winning system of~\newcite{zhang2019no}.

%evaluate our single task BERT model, trained on MICRO-ARA we crawl up to 500 tweets from each of 500 users from the MADAR~\cite{bouamor2019madar_sharedtask} user base and extract the following number of tweets from each user: \textit{\{10, 25, 50, 75, 100, 500\}}. We run our best performing BERT model (from the 21 countries in Table~\ref{tab:sprvsd_eval}) on these user tweets, one tweet at a time. Taking the majority class on each user's tweets, we find that with 100 tweets, for example, the model can reach 65.171\% acc and with 500 tweets, it can reach 66.787\% acc.~\footnote{We provide the full results table for user-level evaluation in supplementary material.}~\footnote{In our 233,105 automatically tagged users, 94.85\% have $>=$100 tweets, suggesting a model based on only 100 tweets would have very high coverage.}
